Why Are Convolutional Nets More Sample-Efficient than Fully-Connected Nets?

Convolutional neural networks often dominate fully-connected counterparts in generalization performance, especially on image classification tasks. This is often explained in terms of 'better inductive bias'. However, this has not been made mathematically rigorous, and the hurdle is that the fully connected net can always simulate the convolutional net (for a fixed task). Thus the training algorithm plays a role. The current work describes a natural task on which a provable sample complexity gap can be shown, for standard training algorithms. We construct a single natural distribution on $\mathbb{R}^d\times\{\pm 1\}$ on which any orthogonal-invariant algorithm (i.e. fully-connected networks trained with most gradient-based methods from gaussian initialization) requires $\Omega(d^2)$ samples to generalize while $O(1)$ samples suffice for convolutional architectures. Furthermore, we demonstrate a single target function, learning which on all possible distributions leads to an $O(1)$ vs $\Omega(d^2/\varepsilon)$ gap. The proof relies on the fact that SGD on fully-connected network is orthogonal equivariant. Similar results are achieved for $\ell_2$ regression and adaptive training algorithms, e.g. Adam and AdaGrad, which are only permutation equivariant.

==> hardness.tex <==
\section{Hardness on learning with equivariant algorithms}\label{sec:lower_bounds}
\vspace{-0.1cm}
In this section, we present our main results on the hardness of learning, each of them consisting a family of (or a single) distribution which is hard for equivariant algorithms, including FC network of any depth and trained by GD, but simple for other non-equivariant algorithms, such as ERM on simple CNNs. \footnote{As a fair comparison, we also provide the convergence analysis of GD on these CNNs in Appendix, though the computational efficiency is not the focus of our paper. Instead, the focus is sample complexity, and being learnable by simple CNNs via ERM is just a natural way to demonstrate the simplicity of the problem itself and the price of  ignoring the problem structure and being equivariant. Note that we are not claiming every 
convolutional architecture has low sample complexity. }  Behind these results are two different views of the impact of equivariance, which are explained in the next two subsections respectively. %, together with the corresponding hardness results. 
Due to space limit, part of the proofs are deferred to Appendix.

\vspace{-0.1cm}
\subsection{View 1: Equivariance confuses the algorithm when samples are few}
\vspace{-0.1cm}
Given training dataset $S_N=(\vX_N,\vy_N) = \nxy$ and test data $(\vx,y)$, 
%the \emph{expected error} of a randomized learning algorithm $\cA$, $\err_\cA(\cS_N,(\vx,y))$ is defined as $\prob{}{\cA(\cS_N)(\vx)=y}$, where the probability is taken over the internal randomness of $\cA$. 
%For convenience, we also denote the above error by $\err_\cA(\cbS)$, where $\cbS = (\vbX,\vby) = \nbxy$. Therefore, the expected error of algorithm $\cA$ on learning distribution $P$ with $n$ samples is $\Exp{\cbS\sim P^{n+1}}{\err_\cA(\cbS)}= \Exp{\vx_i,y_i\sim P}{\err_\cA(\nbxy)}$. 
by definition of $\cG_\cX$-equivariant algorithms(Algorihtm~\ref{alg:iter}), we have 
\vspace{-0.1cm}
\begin{equation}\label{eq:output_equiv}
[\cA(\vX_N,\vy_N)](\vx)\distequal [\cA(g(\vX_N),\vy_N)](g(\vx)),\ \forall g \in \cG_\cX
\end{equation}	
 meaning that the prediction of the learning algorithm made on unseen data only depends on the orbit of the dataset lies in,  $\{(g(\vX_N),g(\vx))| g\in \cG_\cX\}$, as well as the labels, $\vy$.
%Similarly, we have 
% \begin{equation}\label{eq:output_equiv}
%\err_\cA(\vbX,\vby) = \err_\cA(g(\vbX),\vby),\forall g\in\cG.  	
% \end{equation}

Thus the first view is that $\cG_\cX$-equivariance can confuse $\cA$ with unseen data of different labels when training data are few, as illustrated in the warm-up example. Because when $n$ is small,  with high probability we could find a $g\in \cG_\cX$, such that the training dataset is invariant under transformation $g$, $g(\vX_N)=\vX_N$, but many test data changes, from $\vx$ to $g(\vx)$, where $\vx$ and $g(\vx)$ have different labels. However $\cG_\cX$-equivariance implies $\cA$ has to make the same prediction for $\vx$ and $g(\vx)$, thus resulting in large test error. Below we will show how Equation~\ref{eq:output_equiv} forbids any permutation equivariant algorithm $\cA$ to learn a single task  with $O(d)$ samples.


%\zhiyuan{To be turned into a warm-up}
%\begin{thm}
%	There's a single task $\cP=\{P\}$, such that for any orthogonal-equivariant algorithm $\cA$, $\cN(\cA,\cP,\frac{1}{8},\frac{1}{8})\ge \cN^*(\cA,\cP,\frac{1}{4})\ge \frac{d}{2}$.
%\end{thm}


%\begin{proof}
%	We construct $P$ as the uniform distribution on $ \{(\ve_i y,y)| i\in\{1,2,\ldots,d\}, y=\pm1\}\subseteq \cX\times \cY$. %We further define a 1-1 map $\sigma:\cX \to \cX$, $\sigma(\vx) = -\vx$. One can verify that $P$ is invariant under $\sigma$, namely $P = P\circ\sigma$.
	
%	Suppose $n\leq\frac{d}{2}$, given any $\vX_N,\vy_N$,  regardless the randomness in $\cA$, we have 
	
%	\begin{equation}
%	\begin{split}
%		  &\err_P(\cA(\vX_N,\vy_N))\\
%		= &\prob{\vx,y}{\cA(\vX_N,\vy_N)(\vx)\neq y} \\
%		\ge &\prob{\vx,y}{\cA(\vX_N,\vy_N)(\vx)\neq y \mid \vx^\top\vx_i=0,\forall i}\cdot \prob{}{\vx^\top\vx_i=0,\forall i}\\
%		\ge &\frac{1}{2}\prob{\vx,y}{\cA(\vX_N,\vy_N)(\vx)\neq y \mid \vx^\top\vx_i=0,\forall i}\\
%		= &\frac{1}{4}\prob{\vx,y}{\cA(\vX_N,\vy_N)(\vx)\neq y \mid \vx^\top\vx_i=0,\forall i} \\
%		&+\frac{1}{4}\prob{\vx,y}{\cA((I-2\vx\vx^\top)\vX_N),\vy_N)((I-2\vx\vx^\top)\vx)\neq y \mid \vx^\top\vx_i=0,\forall i}\\
%		= &\frac{1}{4}\prob{\vx,y}{\cA(\vX_N,\vy_N)(\vx)\neq y \mid \vx^\top\vx_i=0,\forall i} \\
%		&+\frac{1}{4}\prob{\vx,y}{\cA(\vX_N),\vy_N)(-\vx)\neq y \mid \vx^\top\vx_i=0,\forall i}\\
%		= &\frac{1}{4}\prob{\vx,y}{\cA(\vX_N,\vy_N)(\vx)\neq y \mid \vx^\top\vx_i=0,\forall i} \\
%		&+\frac{1}{4}\prob{\vx,y}{\cA(\vX_N),\vy_N)(\vx)\neq -y \mid \vx^\top\vx_i=0,\forall i}\\
%		=&\frac{1}{4}
%	\end{split}
%	\end{equation}
%	
%\end{proof}
%\zhiyuan{To be turned into a warm-up}
 %, which means $\err_\cA$ is only a function of the equivalent class $\{(g(\vbX),\vby)| g\in G\}$.

\begin{thm}\label{thm:permutation}
There's a single task $\cP=\{P\}$, such that for any permutation equivariant algorithm $\cA$, $\cN(\cA,\cP,\frac{1}{8},\frac{1}{8})\ge \cN^*(\cA,\cP,\frac{1}{4})\ge \frac{d}{10}$. Meanwhile,  $\cN(\erm_{CNN},\cP,0,\delta) \le \log_2{\frac{1}{\delta}}+2$, where   $\erm_{CNN}$ stands for $\erm_{CNN}$ for function class of 2-layer CNNs.
\end{thm}

\begin{proof}
	We consider two types of local textures in a 1-dimensional image with $d$ pixels, namely $\reals^d$ --- we define $\vt_i =\ve_i+\ve_{i+1}$ and $\vs_i = \ve_i+\ve_{i+2}$. We now construct the distribution $P$ as the uniform distribution on $\{(\vs_i,1)\}_{i=1}^n\cup\{(\vt_i,-1)\}_{i=1}^n$. 
	
	\textbf{Lower Bound:} We further define permutation $g_i$ as $g_i(\vx) = \vx - (\ve_{i+1}-\ve_{i+2})^\top(  \ve_{i+1} -\ve_{i+2})\vx$. Clearly, $g_i(\vt_i) = \vs_i, g_i(\vs_i) = \vt_i$. For $i,j\in\{1,2,\ldots,d\}$, we define $d(i,j) = \min\{(i-j) \textrm{ mod } d, (j-i) \textrm{ mod } d\}$. It can be verified that if $d(i,j)\ge 3$, then $\tau_i(\vs_j) = \vs_j, \tau_i(\vt_j) = \vt_j$. For $\vx=\vs_i$ or $\vt_i$, $\vx'=\vs_j$ or $\vt_j$, we define $d(\vx,\vx') = d(i,j)$.
	
	Given $\vX_N,\vy_n$, we have 
%	\begin{equation}
%		\begin{split}
$			\prob{}{B}:=\prob{\vx}{ d(\vx,\vx_i)\ge 3,\ \forall i} \ge \frac{d-\frac{d}{10}*5}{d} =\frac{1}{2}.$
%		\end{split}
%	\end{equation}
Therefore, we have 
	\begin{equation*}
	\begin{split}
		  &\err_P(\cA(\vX_N,\vy_N)) = \prob{\vx,y,\cA}{\cA(\vX_N,\vy_N)(\vx)\neq y} \ge \prob{\vx,y,\cA}{\cA(\vX_N,\vy_N)(\vx)\neq y\mid B}\prob{}{B}\\
		  &\ge  \frac{1}{2}\prob{\vx,y,\cA}{\cA(\vX_N,\vy_N)(\vx)\neq y\mid B}\\
		  & = \frac{1}{4}\prob{i,\cA}{\cA(\vX_N,\vy_N)(\vs_i)\neq 1\mid B}  + \frac{1}{4}\prob{i,\cA}{\cA(\vX_N,\vy_N)(\vt_i)\neq -1\mid B} \\
  		  &\overset{(\ref{eq:output_equiv})}{=} \frac{1}{4}\prob{i,\cA}{\cA(\tau_i(\vX_N),\vy_N)(\tau_i(\vs_i))\neq 1\mid B}  
		  + \frac{1}{4}\prob{i,\cA}{\cA(\vX_N,\vy_N)(\vt_i)\neq -1\mid B} \\
		  &= \frac{1}{4}\prob{i,\cA}{\cA(\vX_N,\vy_N)(\vt_i)\neq 1\mid B}  + \frac{1}{4}\prob{i,\cA}{\cA(\vX_N,\vy_N)(\vt_i)\neq -1\mid B} =\frac{1}{4}.
	\end{split}
	\end{equation*}

	Thus for any permutation equivariant algorithm $\cA$, $\cN^*(\cA,\{P\},\frac{1}{4})\ge\frac{d}{10}$.
\end{proof}

\begin{remark}
For proof simplicity, we take texture of length 2 as an illustrative example. The constructed task resembles edge detection problems with an image gradient operator~\cite{sobel19683x3}. It is straightforward to extend the same proof to more sophisticated local patterns of any constant length and to 2-dimensional images.
\end{remark}

\subsection{View 2: Learning a more complex problem}

In this section, two results are presented in two different settings. For the first result, we consider the setting where there's a unique input distribution a priori. By allowing a class of hypotheses instead of a single hypothesis, we can show a $\tilde{\Omega}(d^2)$ vs $O(d)$ sample complexity separation between equivariant algorithms and the others, such as \erm\  on CNN.  Second, following the setting of \cite{ng2004feature}, where all possible input distributions are allowed, we get a stronger separation result than \cite{ng2004feature}, $\Omega(d^2)$ vs $O(1)$, between orthogonal equivariant algorithms and the others, such as \erm \  on CNN.

%It's often inconvenient to work with algorithmic properties, such as equivariance. In this subsection we present a new  reduction from standard PAC learning with a more complex problem to the original equivariant learning problem. This reduction is tight if the $\cG_\cX$ is compact, and would make the lower bounds conceptually easier. 

Given $\cG_\cX$-equivariant algorithm $\cA$, by definition,   $\cN^*(\cA,\cP,\eps)= \cN^*(\cA,\cP \circ g^{-1},\eps),\forall g\in \cG_\cX$.
%where $\cP\circ g^{-1}$ is defined as $\{P\circ g^{-1}| \forall P \in \cP\}$. 
Consequently, we have  
\begin{equation}\label{eq:augment_problem}
%\cN(\cA,\cP,\eps,\delta)= \cN(\cA,\bigcup\limits_{g\in \cG_\cX}\cP\circ g^{-1},\eps,\delta).	
\cN^*(\cA,\cP,\eps)= \cN^*(\cA,\cP\circ \cG_\cX,\eps).	
\end{equation}


\begin{lem}\label{lem:reduction}
Let $\mathbb{A}$ be the set of all algorithms and $\mathbb{A}_{\cG_\cX}$ be the set of all $\cG_\cX$-equivariant algorithms, we have 

\begin{equation}\label{eq:inf_augment_problem}
	\inf_{\cA\in \mathbb{A}_{\cG_\cX}}\cN^*(\cA,\cP,\eps) \ge \inf_{\cA\in\mathbb{A}}\cN^*(\cA,\cP\circ \cG_\cX,\eps)
\end{equation}\vspace{-0.1cm}
The equality is attained when $\cG_\cX$ is a compact group.
\end{lem}






\begin{thm}\label{thm:augment_function}
Suppose  $\cP_\cX$ is invariant under group $\cG_\cX$, i.e., $\cP_\cX\circ\cG_\cX = \cP_\cX$, we have 
\begin{equation}\label{eq:augment_function}
	\inf_{\cA\in \mathbb{A}_{\cG_\cX}}\cN^*(\cA,\cP_\cX\diamond \cH,\eps) \ge \inf_{\cA\in\mathbb{A}}\cN^*(\cA,\cP_\cX\diamond (\cH\circ\cG_\cX),\eps) 
\end{equation}

The equality is attained when $\cG_\cX$ is a compact group.
\end{thm}

\begin{proof}
	Simply note that $ (\cP_\cX \diamond \cH)\circ \cG_\cX= (\cP_\cX\circ \cG_\cX) \diamond (\cH\circ \cG_\cX) =\cP_\cX\diamond (\cH\circ\cG_\cX)$, the theorem is immediate from Lemma~\ref{lem:reduction}.
\end{proof}

\begin{remark}
The sample complexity in standard PAC learning is usually defined over all the possible input distributions. In that case, $\cP_\cX$ is always invariant under group $\cG_\cX$, and thus Theorem~\ref{thm:augment_function} implies that PAC learning a hypothesis class $\cH$ for an $\cG_\cX$-equivariant algorithm is as hard as learning $\cH\circ \cG_\cX$ without equivariance constraint. To the best of our knowledge, this lemma is first result to prove hardness in sample complexity for single hypothesis learning via algorithmic restriction.
\end{remark}

As a direct application of the above Theorem~\ref{thm:augment_function}, we have the following two theorems.



\begin{thm}\label{thm:single_dist}
	There is a problem with single input distribution, $\cP = \{P_\cX\}\diamond \cH$, and a constant $\eps_0 >0$,  such that for any orthogonal equivariant algorithms $\cA$, $\cN^*(\cA, \cP, \eps_0 ) = \tilde{\Omega}(d^2)$, while there's a 2-layer CNN architecture, such that $\cN(\erm_{CNN},\cP,\eps,\delta) = O(\frac{d\log\frac{1}{\eps}+\log\frac{1}{\delta}}{\eps})$.
\end{thm}

\begin{proof}[Proof of Theorem~\ref{thm:single_dist}]
	\textbf{Sketch for lower bound:} Let $\cP = \{N(0,I_d)\}\diamond \cH$, where $\cH = \{ \sign{\sum_{i=1}^d \alpha_i x_i^2}\mid \alpha_i\in\reals\}$. Since $N(0,I_d)$ is invariant under all orthogonal transformations, by Theorem~\ref{thm:augment_function}, $\cN^*(\cA, \cP, \eps_0 ) = \cN^*(\cA, {N(0,I_d)}\diamond(\cH \circ \cO(d)) , \eps_0 )$. Furthermore, it can be show that $\cH \circ \cO(d)= \{\sign{\sum_{i,j}\beta_{ij}x_ix_j}\mid \beta_{ij}\in \reals\}$, which is the sign functions of all quadratics in $\reals^d$. Thus we've reduced the problem of learning sign of any quadratic function to learning $\cH$ with orthogonal equivariant algorithms.
	
		Next we show learning quadratic functions on Gaussian input distribution needs $\Omega(d^2)$ samples for any algorithm (see Lemma~\ref{lem:lb_quadratic} and the proof is postponed to Appendix~\ref{sec:proofs}). 	

	\begin{lem}\label{lem:lb_quadratic}
		Let $\cH = \{\sign{ \vx^\top A\vx]| \forall A\in \reals^{d\times d}}\}$, it holds that for any algorithm $\cA$, for sufficiently large $d$, there's a constant $\eps_0 >0$, such that 

		 \[\cN^*(\cA, \{N(0,I_d)\}\diamond \cH, \eps_0 ) = \Omega(\frac{d^2}{\log^2d}).\]	

	\end{lem}	
	The intuition here is we can pick a distribution over all quadratic functions, say $\beta_{ij}\overset{i.i.d.}{\sim} N(0,1)$, such that with high probability, conditioned on all the training data and their labels, the label of any fixed unseen data still remains random, and thus no algorithm could achieve $o(1)$ error.

\end{proof}

\begin{rem}
	Theorem~\ref{thm:single_dist} could be extended to the case of regression (real number output) naturally.
\end{rem}

\begin{thm}\label{thm:single_function}
	There is a problem with single hypothesis, $\cP = \cP_\cX \diamond \{h^*\}$, such that for any rotaion equivariant algorithms $\cA$, $\cN^*(\cA, \cP, \frac{1}{4}) = \Omega(d^2)$, while there's a 2-layer CNN architecture, such that $\cN(\erm_{CNN},\cP,\eps,\delta) = O\left(\frac{1}{\eps}\left( \log\frac{1}{\eps}+ \log\frac{1}{\delta})\right)\right)$.
\end{thm}




==> intro.tex <==
\section{Introduction}
\label{sec:intro}
\vspace{-0.1cm}
Deep convoluitonal architectures are the initiator of the current deep learning revolution and continue to be the mainstay~\cite{krizhevsky2012imagenet,he2016deep, huang2017densely}. It is a consensus among practitioners that convolutional neural nets generalize significantly better their fully-connected counterparts on any task where translation invariance is inherent, i.e. ImageNet, CIFAR10. Common explanations include convolutional architectures have better \textquotedblleft inductive bias\textquotedblright or they have less total number of parameters. However, a formal theoretical treatment is still largely missing, even in the minimal case where the task can be solved by learning a single convolutional filter, e.g. edge detection or texture classification.

Providing mathematically rigorous explanation for such an empirical generalization performance gap is challenging. First of all this requires showing an upper bound of convolutional nets and a lower bound of fully-connected on the \emph{same} task simultaneously. Most well-developed techniques for lower-bounding sample complexity (i.e. PAC learning lower bounds) rely on constructing \emph{a family of tasks} and showing, for any learning algorithm, there must exist a corresponding task in the family that fails it. These techniques usually allow the learning algorithms to be arbitrary, however, in our case, if we do not account for the properties of learning algorithms, this sample complexity separation between convolutional and fully-connected nets would not even exist. This is because, on a fixed task, we can always hypothetically construct a learning algorithm for fully-connected nets that trivially simulates the optimal convolutional net, and thus the gap would be zero. Thus utilizing properties of learning algorithms will be necessary in proving this type of separation.

 One major property of SGD for fully-connected nets  is that no matter how deep and wide the network is and what the learning schedules are, SGD is inevitably \emph{orthogonal-equivariant}\textemdash\textemdash the learnt nets will have the same test loss even if any orthogonal transformation is applied to coordinates of training and test examples. \cite{ng2004feature} (within which it is named ``orthogonal invariant'' instead) proved $\Omega(d)$ versus $O(1)$ sample complexity separation between orthogonal equivariant algorithms  and other algorithms for learning a single linear threshhold function for all distributions. We improve this result in the following two sense: (1). we show $\Omega(d^2)$ vs $O(1)$ separation; (2). our lower bound holds even for a single target function with a single fixed distribution. 
 
 Towards this result, we propose a general approach to reduce certain PAC learning problem to learning with equivariant algorithms. The high-level idea is that if there's an equivariant algorithm which learns the joint distribution, then the same algorithm learns all the joint distributions achieved by rotating the input distribution. In the meantime, the convolutional structure breaks the symmetry and frees learning algorithms from the confusion. In this way we formally provide \emph{algorithmic symmetry} as an answer to the question posed in the title.

 However, orthogonal equivariance is  less common than permutation equivariance in deep learning, as the former one excludes popular adaptive algorithms such as AdaGrad and Adam, $\ell_1$ regularizer, and non-spherical symmetric initialization methods like uniform distribution. We demonstrate a \emph{single} and \emph{natural} task on $\R^d\times\{\pm 1\}$ that resembles real-life image texture classification, on which we prove any permutation-invariant learning algorithm requires $\Omega(d)$ training examples to generalize, while Empirical Risk Minimization with $O(1)$ examples suffice to learn a convolutional net eschewing from \emph{the curse of symmetry}. Essentially, any permutation invariant algorithm will be confused with permutations of the coordinates, if not observing enough training examples.  


\textbf{Paper structure.} In Section~\ref{sec:related} we discuss about related works. In section~\ref{sec:notation}, we define the notation and terminologies. In Section~\ref{sec:equiv}, we  define the equivariant algorithms and show that a broad class of gradient-based algorithms are equivariant. In Section~\ref{sec:lower_bounds}, we present our main results on the lower bound of orthogonal(permutation)  equivariant algorithms.
\vspace{-0.1cm}
\paragraph{Our contributions:} In the work, we present the following:
\begin{itemize}[leftmargin=*]
	\item a general sufficient condition for an iterative algorithm to be equivariant (under some group), met by a broad class of popular training algorithms for fully-connected neural networks, such as AdaGrad, SGD with momentum, and Adam, with or without regularizers.
	\item a class of input distributions and a fixed hypothesis which requires $\Omega(d^2/\eps)$ training samples for any orthogonal equivariant algorithms to achieve $O(\eps)$ test error. Meanwhile, CNN learns the hypothesis class with $O(d/\eps)$ samples.
	\item a fixed distributions and a fixed hypothesis which requires $\Omega(d^2)$ training samples for any orthogonal equivariant algorithms to achieve $O(1)$ test error. Meanwhile, CNN learns the hypothesis class with $O(1)$ samples.
	\item a fixed input distribution and a hypothesis class which requires $\Omega(d^2/\eps)$ training samples for any orthogonal equivariant algorithms to achieve $O(\eps)$ test error. Meanwhile, CNN learns the hypothesis class with $O(\eps)$ samples.
	\item a fixed input distribution and a fixed hypothesis  which requires $\Omega(d)$ training samples for any permutation equivariant algorithms to achieve $O(1)$ test error. Meanwhile, CNN learns the hypothesis with only constant samples.
\end{itemize}
\vspace{-0.2cm}
%\Yi{todo: introduce algorithmic symmetry}

==> lowerbound.tex <==

\section{Lower bound on sample complexity for rotation invariant algorithms}
\begin{lem}\label{lem:function_indep}
Functions of independent random variables are independent.
\end{lem}

\begin{lem}\label{lem:anti-concentration}
For any $z>0$, we have 
\begin{align*}
    \Pr_{x\sim N(0,\sigma)}\left(|x|\leq z\right) \leq \frac{2}{\sqrt{\pi}}\frac{z}{\sigma}
\end{align*}
\end{lem}
\begin{proof}
\begin{align*}
 \Pr_{x\sim N(0,\sigma)}\left(|x|\leq z\right) &= \int_{-z}^z \frac{1}{\sqrt{2\pi}~\sigma}\exp\left(-\frac{x^2}{2\sigma^2}\right)\mathrm{d}x\\
 &\leq \sqrt{\frac{2}{\pi}}\frac{z}{\sigma}
\end{align*}
\end{proof}

\begin{lem}\label{lem:projection}
For any fixed subspace $S\in\R^{d^2}$ with dimension $k\leq\frac{d^2}{12\log^2(d/\delta)}$, of which $Q$ is the projection matrix, if $x$ is drawn from $N(0, I_d)$, then we have 
\begin{align*}
    \|Q(x\otimes x)\|_2^2 \leq \frac{1}{3}d^2 + O(d)\\
    \text{and}~~~\|(I-Q)(x\otimes x)\|_2^2 \geq \frac{2}{3}d^2 - O(d)
\end{align*}
with probability over $x_{n+1}$  at least $1-\delta$.
\end{lem}



\begin{proof}
Let $\vec{I}_d$ denote the vectorized representation in space $\R^{d^2}$ of the identity matrix $I_d\in\R^{d\times d}$. Whether the subspace $S$ contains $\vec{I}_d$ affects the projection of $x\otimes x$ onto it. However, without loss of generality, we define $S':=\text{span}(S\cup\{\vec{I}_d\})$ and show it suffices to upper bound the projection onto $S'$ which is strictly larger. We denote $S'$'s dimensionality by $k'$ and note that $k'\leq k+1$. Let $\{e_1, e_2, \ldots, e_{k'}\}$ be an orthonormal basis of $S$ such that $e_{k'}=I_d/\sqrt{d}$. Now we have
\begin{align*}
    (x\otimes x)^\top Q (x\otimes x) = \sum_{i=1}^{k} \left(e_i^\top (x\otimes x)\right)^2
\end{align*}
Note that $e_i^\top \E[x\otimes x]=0$ for $i\in[k'-1]$ and $e_{k'}^\top \E[x\otimes x]=\sqrt{d}$. It follows by Hanson-Wright Inequality and a simple union bound over $e_i$'s that
with probability $\geq 1 - k' \exp(-\min\{t, t^2\})$, we have
\begin{align*}
\forall i\in[k'-1], ~~~|e_i^\top (x\otimes x) | &\leq t, \\
\text{and}~~ |e_{k'}^\top (x\otimes x) | &\leq \sqrt{d} + t 
\end{align*}
If we choose $t=\log(k'/\delta)=O(\log(d/\delta))$, then we have
\begin{align*}
    (x\otimes x)^\top Q (x\otimes x) &\leq k't^2 + d + \sqrt{d} t \\
    &\leq \frac{1}{3}d^2 + O(d)
\end{align*}
with probability at least $1-O(\delta)$, where we use the fact $k\leq\frac{d^2}{12\log^2(d/\delta)}$.
Combining the above result with the fact that $\|x\otimes x\|_2^2=d^2\pm O(d)$ w.h.p., we arrive at the desired conclusion.

\end{proof}


\begin{thm}

\end{thm}
\begin{proof}
Let $S$ denote the span of $\{x_i\otimes x_i\}_{i=1}^n$ and $Q$ is projection matrix onto $S$. We know $\text{dim}(S)\leq n\leq\frac{d^2}{12\log^2(d/\delta)}$. From now on, for notational simplicity, we write $\textit{var}_1:=\|Q(x_{n+1}\otimes x_{n+1})\|_2^2$ and $\textit{var}_2:=\|(I-Q)(x_{n+1}\otimes x_{n+1})\|_2^2$. Now we draw $a\sim N(0, I_{d^2})$
\begin{align*}
    a^\top(x_{n+1}\otimes x_{n+1}) &= \underbrace{a^\top Q(x_{n+1}\otimes x_{n+1})}_{n_1}\\
    &+ \underbrace{a^\top (I-Q)(x_{n+1}\otimes x_{n+1}}_{n_2})
\end{align*}
where $n_1, n_2\in\R$ are two \emph{independent} Gaussian variables, i.e. $n_1\sim N(0, \textit{var}_1)$ and $n_2\sim N(0, \textit{var}_2)$. In fact, the independence follows from the orthogonality between the vectors $Q(x_{n+1}\otimes x_{n+1})$ and $(I-Q)(x_{n+1}\otimes x_{n+1})$. 


By lemma~\ref{lem:projection}, conditioned on $\{x_i\}_{i=1}^n$, we have
\begin{align}\label{ineq: condition}
\frac{\textit{var}_2}{\textit{var}_1} = \frac{\frac{2}{3}d^2 - O(d)}{\frac{1}{3}d^2 + O(d)}\leq 2 - O(1/d)
\end{align}
with probability at least $1-\delta$ over randomness of $x_{n+1}$.

From now on, we condition on the event of Inequality~\ref{ineq: condition} being true, and then fix all the $x_i$'s, leaving $a$ to be the only source of randomness. We call this event $E_1$ and $\Pr(E_1)\geq 1-\delta$.
Note that $\mathcal{A}(S_n)(x_{n+1})$ is a function of $y_i$'s which are in turn functions of $a^\top(x_i\otimes x_i)$'s for $i\in[n]$, i.e.
\begin{align*}
    \mathcal{A}(S_n)(x_{n+1}) &= f(a^\top(x_1\otimes x_1), \ldots, a^\top(x_n\otimes x_n))\\
    &:=f(P_n)
\end{align*}
for some fixed function $f$, where we introduced a new notation $P_n:=\left(a^\top(x_1\otimes x_1), \ldots, a^\top(x_n\otimes x_n)\right)$ to be a tuple of $n$ random variables and $p_n$ to be any realization of $P_n$. 

On the other hand, $n_1=g(P_n)$ for some fixed function $g$ as well. In fact, since $Q(x_{n+1}\otimes x_{n+1})=\sum_{i=1}^n c_i (x_i\otimes x_i)$ for fixed constants $c_i$'s, it clear that $n_1=\sum_{i=1}^n c_i a^\top(x_i\otimes x_i)$. Therefore, conditioned the values of $P_n$ for $i\in[n]$, the values of $n_1$ and $\mathcal{A}(S_n)(x_{n+1})$ are both determined while $n_2$ remains random due to independence.

Now we define a new event 
%$E_2:=\left\{ p_n \middle|~~ |n_1|=|g(p_n)|\leq \sqrt{\textit{var}_1} \right\}$
$E_2:=  |n_1|=|g(P_n)|\leq \sqrt{\textit{var}_1} $
, and we show it occurs with constant probability:
\begin{align*}
    \Pr_a & \left( E_2 \middle|~ E_1 \right) = \Pr_a\left(|n_1|\leq \sqrt{\textit{var}_1} \middle|~ E_1\right) \\
    &= \Pr_{n_1\sim N(0, \textit{var}_1)} \left( |n_1|\leq \sqrt{\textit{var}_1}\right) \geq 1- \frac{\E[|n_1|]}{\sqrt{\textit{var}_1}} \\
    &\geq 1 - \sqrt{\frac{2}{\pi}} \geq 0.2
\end{align*}

Then we are ready to examine the expected population loss of $A(S_n)$,
\begin{align*}
    &~\E_a\E_{x_{n+1}}\left[\mathcal{A}(S_n)(x_{n+1})\not=\mathbb{1}\{a^\top x_{n+1}\geq 0\}\right] \\
    &\geq \int_{x\in E_1}\E_a\left[\mathcal{A}(S_n)(x)\not=\mathbb{1}\{a^\top x \geq 0\}\right] \Pr(x_{n+1}=x)\mathrm{d}x \\
    &\geq (1-\delta) \min_{x\in E_1}\E_a\left[\mathcal{A}(S_n)(x)\not=\mathbb{1}\{a^\top x \geq 0\}\right]
\end{align*}
The above expression can be in turn lower bounded by observing that for all $x\in E_1$, we have 
\begin{align*}
    \E_a & \left[\mathcal{A}(S_n)(x)\not=\mathbb{1}\{a^\top x \geq 0\} \right] \\
    &=\Pr_a\left(\mathcal{A}(S_n)(x)\not=\mathbb{1}\{n_1+n_2\geq0\} \right)\\
    &\geq 0.2 \Pr_a\left(f(P_n)\not=\mathbb{1}\{g(P_n)+n_2\geq0\}\right)
\end{align*}
We now proceed by an important observation that, conditioned on $P_n$ taking value $p_n$ for some $p_n\in E_2$, fixed a value of $p_n$, the randomness of $n_2$ will make $\mathbb{1}\{g(P_n)+n_2\geq0\}$ not match $f(P_n)$ with constant probability. The reasons are the following: ~~1) $f(p_n)$ is fixed as either $+1$ or $-1$, ~~2) $g(f_n)$'s magnitude is at most $\sqrt{\textit{var}_1}$, ~~3) $n_2$ is still a Gaussian random variable (due to independence) and its standard deviation is much larger than $\sqrt{\textit{var}_1}$. With a slight abuse of notation, we denote the \emph{probability density function} of the random variable $P_n$ as $\Pr_a(P_n = \cdot)$. To formalize the observation, we have for all $x\in E_1$, we have for all $x\in E_1$ that
\begin{align*}
    &\Pr_a\left(f(P_n)\not=\mathbb{1}\{g(P_n)+n_2\geq0\} \right)\\
    &= \int_{p_n\in E_2}\Pr_a\left(f(p_n)\not=\mathbb{1}\{g(p_n)+n_2\geq0\}\right)\Pr_a(P_n = p_n)\mathrm{d}p_n\\
    &\geq \frac{1}{2}\int_{p_n\in E_2}\Pr_{a}\left(|n_2| \geq |g(p_n)| \right)\Pr_a(P_n = p_n) \mathrm{d}p_n\\
    &\geq \frac{1}{2}\left(1-\sqrt{\frac{2}{\pi}}\sqrt{\frac{\textit{var}_1}{\textit{var}_2}}\right)\Pr_a\left(P_n\in E_2\right)\\
    &\geq 0.1 \left(1-\sqrt{\frac{1}{\pi}}\right) - O(\frac{1}{d})
\end{align*}
where we used the anti-concentration of Gaussian random variables shown in Lemma~\ref{lem:anti-concentration}.

Putting everything together, we now conclude that if we choose $1-\delta>0.99$, then
\begin{align*}
    \E_a\E_{x_{n+1}}\left[\mathcal{A}(S_n)(x_{n+1})\not=\mathbb{1}\{a^\top x_{n+1}\geq 0\}\right]=\Omega(1)
\end{align*}
which implies there exists an $a^*\in\R^{d^2}$ such that
\begin{align*}
    \E_{x_{n+1}}\left[\mathcal{A}(S_n)(x_{n+1})\not=\mathbb{1}\{{a^*}^\top x_{n+1}\geq 0\}\right]=\Omega(1)
\end{align*}
which is the desired statement.
\end{proof}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> new_intro_conv_task.tex <==
\section{Introduction}
\label{sec:intro}
\vspace{-0.1cm}
Deep convoluitonal architectures are the initiator of the current deep learning revolution and continue to be the mainstay~\cite{krizhevsky2012imagenet,he2016deep, huang2017densely}. It is a consensus among practitioners that convolutional neural nets generalize significantly better their fully-connected counterparts on any task where translation invariance is inherent, i.e. ImageNet, CIFAR10. Since ultra wide fully-connected nets can simulate any convolutional nets of smaller size, this is not an issue of expressiveness. Common explanations include convolutional architectures have better \textquotedblleft inductive bias\textquotedblright or they have less total number of parameters. However, a formal theoretical treatment is still largely missing.

Providing mathematically rigorous explanation for such an empirical generalization performance gap requires showing an upper bound of convolutional nets and a lower bound of fully-connected on the \emph{same} task simultaneously. More specifically, in this work we focus on proving lower bounds for fully-connected neural networks on Conv tasks. \red{ Here a task refers to the combination of an input distribution and a labeling function, or a realizable joint distribution on data and labels.}  and the labeling function of a Conv task can be expressed by small-size convolutional networks (e.g. of constant parameters) thus sample complexity is provably low. The main challenge here is that most well-developed techniques for lower-bounding sample complexity (i.e. PAC learning lower bounds) are \emph{information theoretic} and disregard the properties of the algorithm.
%, i.e. for any learning algorithm, there must exist a corresponding task in the constructed family of tasks that fails it. 
However, in our case, if we do not account for the properties of learning algorithms, this sample complexity separation between convolutional and fully-connected nets would not even exist. This is because we can always hypothetically construct a learning algorithm for fully-connected nets that trivially simulates the optimal convolutional net, and thus the gap would be zero. Thus utilizing properties of learning algorithms will be essential in proving this type of separation.

\begin{figure}[h]
\includegraphics[width=14cm, height=5cm]{figures/fc_vs_cnn.pdf}
\caption{Illustration of generalization performance of convolutional versus fully-connected models trained by SGD. Here the input data are $3\times32\times32$ three-channel images and the binary label indicates for each image whether the first channel has larger $\ell_2$ norm than the second one. The input images are drawn from entry-wise independent Gaussian (left) and CIFAR-10 (right). In both cases, the convolutional net consists of a $3\times 3$ convolution with $10$ hidden channel + quadratic activation + $3\times 3$ convoluiton with a single output channel + global average pooling, and the fully-connected net consists of a fully-connected layer with 3072 hidden nodes + quadratic activation + a fully-connected layer with a single node.}
\vspace{-0.2cm}
\label{fig:fc_vs_cnn}
\end{figure}




One major property of SGD for fully-connected nets \emph{orthogonal-equivariance}, no matter how deep and wide the networks are and what the learning schedules are \textemdash\textemdash the learnt nets will make the same predictions even if an orthogonal transformation is simultaneously applied to training and test examples. \cite{ng2004feature} (within which it is named ``orthogonal invariant'' instead) proved that,  for a family of tasks (all possible input distributions and a single fixed linear threshold function), logistic regression with $\ell_1$ regularization only needs $O(1)$ samples for each task, while for any orthogonal equivariant algorithm, there's a task in this family requires $\Omega(d)$ samples to learn.
% $\Omega(d)$ versus $O(1)$ sample complexity separation between orthogonal equivariant algorithms  and logistic regression with $\ell_1$ regularization for learning a single linear threshhold function for all distributions.  
  We improve this result in the following two senses: 
(1) we prove $\Omega(d^2)$ vs $O(1)$ separation; (2) we prove lower bounds for all fully-connected netowrks on a single natural Conv task, i.e., a single target function (sign of $\sum_{i=1}^{d/2} x_i^2 -\sum_{i=d/2+1}^{d}x_i^2$) with a single distribution, the $d$-dimensional Gaussian distribution $N(0,I_d)$. 

Here we highlight that the separation for single natural task better captures the gap between convolutional and fully-connected nets observed in practice, because standard PAC learning lower bounds (also \citep{ng2004feature}) only asserts the existence of a hard (and potentially artificial) distribution for each orthogonal equivariant algorithm, but not for all orthogonal equivariant algorithms. Thus that type of result is not able to explain  why the separation would exist for real-life tasks and that why in practice all fully-connected networks can perform poorly on a single vision task. In contrast, our lower bound  on gaussian distribution and quadratic functions hold simultaneously for all fully-connected networks, and the proof technique also informs us what tasks are hard for orthogonal equivariant algorithms.  In figure~\ref{fig:fc_vs_cnn}, we demonstrate such a gap predicted by our theory (\Cref{thm:1vsdsq_fixed}), i.e. when the data distribution is gaussian, every fully-connected nets must suffer constant loss, with less than $O(d^2)\approx 10^6$ samples, where $d=32\times 32$ is the number of the pixels per image. 

 Towards this result, we propose a general approach to reduce certain PAC learning problem to learning with equivariant algorithms. The high-level idea is that if there's an equivariant algorithm which learns the joint distribution, then the same algorithm learns all the joint distributions achieved by rotating the input distribution. In the meantime, the convolutional structure breaks the symmetry. In this way we formally provide \emph{algorithmic symmetry} as an answer to the question posed in the title. 

 Still, orthogonal equivariance is  less common than permutation equivariance in deep learning, as the former one excludes popular adaptive algorithms such as AdaGrad and Adam, $\ell_1$ regularizer, and non-spherical symmetric initialization methods like uniform distribution. We demonstrate a \emph{single} and \emph{natural} task on $\R^d\times\{\pm 1\}$ that resembles real-life image texture classification, on which we prove any permutation-invariant learning algorithm requires $\Omega(d)$ training examples to generalize, while Empirical Risk Minimization with $O(1)$ examples suffice to learn a convolutional net.


\textbf{Paper structure.} In Section~\ref{sec:related} we discuss about related works. In \Cref{sec:warmup}, we give a warmup example illustrating why equivariance could lead to non-trivial lower bounds even on trivial tasks. In section~\ref{sec:notation}, we define the notation and terminologies, and give a brief  review for some upper and lower bounds for sample complexity.  In Section~\ref{sec:equiv}, we  define the equivariant algorithms and show that a broad class of gradient-based algorithms are equivariant. In Section~\ref{sec:lower_bounds}, we present our main results on the lower bound of orthogonal(permutation)  equivariant algorithms.
\vspace{-0.1cm}
\paragraph{Our contributions:} In the work, we present the following:
\begin{itemize}[leftmargin=*]
	\item a general sufficient condition (\Cref{thm:main_equivariance}) for an iterative algorithm to be equivariant (under some group), met by a broad class of popular training algorithms for fully-connected neural networks, such as AdaGrad, SGD with momentum, and Adam, with or without regularizers. 
	\item a class of input distributions and a fixed hypothesis which requires $\Omega(d^2/\eps)$ training samples for any orthogonal equivariant algorithms to achieve $O(\eps)$ test error. Meanwhile, CNN learns the hypothesis class with $O(1/\eps)$ samples. (\Cref{thm:single_function})
	\item a fixed distributions and a fixed hypothesis which requires $\Omega(d^2)$ training samples for any orthogonal equivariant algorithms to achieve $O(1)$ test error. Meanwhile, CNN learns the hypothesis class with $O(1)$ samples. (\Cref{thm:1vsdsq_fixed})
	\item a fixed input distribution and a hypothesis class which requires $\Omega(d^2/\eps)$ training samples for any orthogonal equivariant algorithms to achieve $O(\eps)$ test error. Meanwhile, CNN learns the hypothesis class with $O(d/\eps)$ samples. (\Cref{thm:single_dist_multi_function}) We also prove an $\ell_2$ regression analog for this $\Omega(d^2)$ vs $\O(d)$ separation, where labels are real-valued instead of binary. (\Cref{thm:regression_single_dist_multi_function})
	\item a fixed input distribution and a fixed hypothesis  which requires $\Omega(d)$ training samples for any permutation equivariant algorithms to achieve $O(1)$ test error. Meanwhile, CNN learns the hypothesis with only constant samples. (\Cref{thm:permutation})
\end{itemize}
\vspace{-0.2cm}
%\Yi{todo: introduce algorithmic symmetry}

==> open.tex <==
We leave it as an open problem to find a single task $\cP=\{P\}$, such that for any orthogonal equivariant algorithm $\cA$ and $\eps >0$, it takes $\Omega(d^2/\eps)$ samples to guarantee the expected error is smaller than $\eps$. In other words, $\cN^*(\cA,\{P\},\eps)=\Omega(d^2/\eps)$. In this work we've shown an $\Omega(d^2 {\eps}^{-\frac{1}{2}+\frac{1}{2d}})$ in \Cref{thm:1vsdsq_fixed} but the rate of $\eps$ is not optimal. We suspect the same construction  actually have an $\Omega(d^2/\eps)$ sample complexity lower bound but the Long's improved version of Benedek-Itai's bound is not tight.

==> warmup.tex <==
\section{Warmup: a $\Omega(d)$ lower bound against orthogonal equivariant algorithms}
\label{sec:warmup}

We start with a simple but insightful example to showcase the main ideas of our techniques. Formal definitions and terminologies can be found in the next section and are not the concern of this section.

We consider a task on $\R^{d}\times\{\pm1\}$ which is a uniform distribution on the set $\{(\ve_i y,y)| i\in\{1,2,\ldots,d\}, y=\pm1\}$, denoted by $P$. Each sample from $P$ is a one-hot vector in $\R^d$ and the sign of the non-zero coordinate determines its label. Now imagine our goal is to learn this task using an algorithm $\mathcal{A}$. After observing a training set of $n$ labeled points $S:=\{(\vx_i,y_i)\}_{i=1}^n$, the algorithm is asked to make a prediction on an unseen test data $\vx$, i.e., $\mathcal{A}(S)(\vx)$. Here we are concerned with \emph{orthogonal equivariant} algorithms \textemdash\textemdash the prediction of the algorithm on the test point remains the same even if we rotate every $x_i$ and the test point $x$ by any orthogonal matrix $R$, i.e., 
\begin{align*}
    \mathcal{A}(\{(R \vx_i,y_i)\}_{i=1}^n)(R \vx) = \mathcal{A}(\{(\vx_i,y_i)\}_{i=1}^n)(\vx)
\end{align*}

As an example, the algorithm can be thought as learning a fully-connected net with gradient descent with possibly $\ell_2$ regularization starting from a Gaussian initialization\footnote{randomization due to initialization will be dealt with formally later. For now we assume the algorithm is deterministic.}. Now we show this algorithm fails to generalize on task $P$, if it observes only $d/2$ training examples. The main idea here is that, for a fixed training set $S$, the prediction $\mathcal{A}(\{(\vx_i,y_i)\}_{i=1}^n)(\vx)$ is determined solely by the inner products bewteen $\vx$ and $\vx_i$'s due to orthogonal equivariance, i.e., there exists a fixed function $f$ (which may depend on $S$) such that\footnote{this can be made formal using the fact that Gram matrix determine a set of vectors up to an orthogonal transformation.}
\begin{align*}
\mathcal{A}(\{(\vx_i,y_i)\}_{i=1}^n)(\vx) = f(\vx^\top\vx_1, \ldots, \vx^\top\vx_n)
\end{align*}
Because $n<d/2$, with probability at least $1/2$ over the random draw of $(\vx, y)\sim P$, $\vx$ will fail to overlap with any point in $S$. This will leave the prediction of $\mathcal{A}$ as a constant $f(0,\ldots,0)$ no matter what $y$'s value will be, marking $\mathcal{A}$'s failure to generalize.


